Compile-Time Java Stream Fusion via mapMulti

The Java Stream API, introduced in Java 8, makes data processing more expressive and concise compared to imperative loops. However, this abstraction can come with significant performance overhead, often due to the creation of multiple intermediate objects during pipeline execution. In functional languages such as Haskell, this problem is addressed through stream fusion, a compile-time optimization that eliminates unnecessary intermediate structures. Inspired by this idea, Streamliner was the first tool to perform ahead-of-time, bytecode-to-bytecode stream optimization for Java by unrolling stream pipelines into imperative loops. In this paper, we introduce an open-source optimizer that takes a different approach. Instead of unrolling streams into loops, it merges consecutive map() and filter() operations into a single mapMulti() call, available since Java 16. Our method avoids several limitations of Streamliner, including its sensitivity to escaping objects in lambda expressions and its restrictions on assigning or passing streams as variables. We evaluated our optimizer on nine benchmarks and observed superior performance in two cases and comparable results in most others. We also applied it to the bytecode of Apache Kafka, successfully executing all 31,799 unit tests without failures.

==> _eolang/paper/056EC3E8B06499C82F27ED78B639A9CA-96-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.23.0
% There are 7 chars in the input: _eolang/paper/056EC3E8B06499C82F27ED78B639A9CA-96-phiq.tex
% ---
% Q.class
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{class}}{}\)\endinput

==> _eolang/paper/056EC3E8B06499C82F27ED78B639A9CA-96-phiq.tex <==
Q.class

==> _eolang/paper/13B5333C7BDB3AAF6B46F89D8794FD92-20-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.23.0
% There are 239 chars in the input: _eolang/paper/13B5333C7BDB3AAF6B46F89D8794FD92-20-phiquation.tex
% ---
%  [[ B_1, name -> e_1, B_2 ]] \longrightarrow [[ B_1, name -> e_2, B_2 ]]
%    \qquad\qquad\text{when}\quad |matches| {(} |"\char94Nums\textdollar{}"| {,} e_1 {)}
%    \qquad\qquad\text{where}\quad e_2 := |concat| {(} |"Op"| {,} |name| {)} {.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} B_1\phiTerminal{,}\; \textnormal{\texttt{name}}{} \mathbin{\phiTerminal{\mapsto}} e_1\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} \longrightarrow \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \textnormal{\texttt{name}}{} \mathbin{\phiTerminal{\mapsto}} e_2\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}}\phiEOL{}
& \quad{} \qquad\qquad\text{when}\quad \textnormal{\texttt{matches}}{} {(} \textnormal{\texttt{"\char94Nums\textdollar{}"}}{} {,} e_1 {)}\phiEOL{}
& \quad{} \qquad\qquad\text{where}\quad e_2 \mathrel{\vDash} \textnormal{\texttt{concat}}{} {(} \textnormal{\texttt{"Op"}}{} {,} \textnormal{\texttt{name}}{} {)} {.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/13B5333C7BDB3AAF6B46F89D8794FD92-20-phiquation.tex <==
 [[ B_1, name -> e_1, B_2 ]] \longrightarrow [[ B_1, name -> e_2, B_2 ]]
   \qquad\qquad\text{when}\quad |matches| {(} |"\char94Nums\textdollar{}"| {,} e_1 {)}
   \qquad\qquad\text{where}\quad e_2 := |concat| {(} |"Op"| {,} |name| {)} {.}


==> _eolang/paper/17A7E27231B5A00DC5BDF9B34BE4AA80-96-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.23.0
% There are 8 chars in the input: _eolang/paper/17A7E27231B5A00DC5BDF9B34BE4AA80-96-phiq.tex
% ---
% Q.method
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{method}}{}\)\endinput

==> _eolang/paper/17A7E27231B5A00DC5BDF9B34BE4AA80-96-phiq.tex <==
Q.method

==> _eolang/paper/300463D412ED4C542835203D66144112-13-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.23.0
% There are 112 chars in the input: _eolang/paper/300463D412ED4C542835203D66144112-13-phiquation.tex
% ---
%  \frg{pattern}{ [[ B_1, @ -> Q.imul, B_2 ]] } \longrightarrow \frg{replacement}{ [[ B_1, @ -> Q.iadd, B_2 ]] }.
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\frg{pattern}{ \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{imul}}{}\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} } \longrightarrow \frg{replacement}{ \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{iadd}}{}\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} }\phiTerminal{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/300463D412ED4C542835203D66144112-13-phiquation.tex <==
 \frg{pattern}{ [[ B_1, @ -> Q.imul, B_2 ]] } \longrightarrow \frg{replacement}{ [[ B_1, @ -> Q.iadd, B_2 ]] }.


==> _eolang/paper/8629FAA36B44FD784C11DFBB19BD9D30-86-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.23.0
% There are 557 chars in the input: _eolang/paper/8629FAA36B44FD784C11DFBB19BD9D30-86-phiquation.tex
% ---
% [[ |j\textdollar{}Numbers| -> [[
%   @ -> Q.class,
%   version -> 61,
%   access -> 33,
%   supername ->
%     "java/lang/Object",
%   interfaces -> [[ ]],
%   |j\textdollar{}object\char64init\char64| -> [[\dots]],
%   |j\textdollar{}total| -> [[\dots]],
%   |\highlight{j\textdollar{}total\textdollar{}0}| -> [[
%     @ -> Q.method,
%     access -> 4106,
%     descriptor -> "(I)I",
%     body -> [[
%       @ -> Q.seq.of6,
%       i2 -> [[ @ -> Q.iload, |v| -> 0 ]],
%       i3 -> [[ @ -> Q.iload, |v| -> 0 ]],
%       i4 -> [[ @ -> Q.imul ]],
%       i5 -> [[ @ -> Q.ireturn ]] ]] ]] ]] ]]
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{j\textdollar{}Numbers}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiEOL{}
& \quad{}\phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{class}}{}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{version}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{61}}{}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{access}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{33}}{}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{supername}}{} \mathbin{\phiTerminal{\mapsto}}\phiEOL{}
& \quad{} \quad{}\textnormal{\texttt{"java/lang/Object"}}{}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{interfaces}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\rrbracket{}}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{j\textdollar{}object\char64init\char64}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\dots\phiTerminal{\rrbracket{}}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{j\textdollar{}total}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\dots\phiTerminal{\rrbracket{}}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{\highlight{j\textdollar{}total\textdollar{}0}}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiEOL{}
& \quad{} \quad{}\phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{method}}{}\phiTerminal{,}\;\phiEOL{}
& \quad{} \quad{}\textnormal{\texttt{access}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{4106}}{}\phiTerminal{,}\;\phiEOL{}
& \quad{} \quad{}\textnormal{\texttt{descriptor}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{"\phiTerminal{(}I\phiTerminal{)}I"}}{}\phiTerminal{,}\;\phiEOL{}
& \quad{} \quad{}\textnormal{\texttt{body}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiEOL{}
& \quad{} \quad{} \quad{}\phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{seq}}{}\phiTerminal{.}\textnormal{\texttt{of6}}{}\phiTerminal{,}\;\phiEOL{}
& \quad{} \quad{} \quad{}\textnormal{\texttt{i2}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{iload}}{}\phiTerminal{,}\; \textnormal{\texttt{v}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{0}}{} \phiTerminal{\rrbracket{}}\phiTerminal{,}\;\phiEOL{}
& \quad{} \quad{} \quad{}\textnormal{\texttt{i3}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{iload}}{}\phiTerminal{,}\; \textnormal{\texttt{v}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{0}}{} \phiTerminal{\rrbracket{}}\phiTerminal{,}\;\phiEOL{}
& \quad{} \quad{} \quad{}\textnormal{\texttt{i4}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{imul}}{} \phiTerminal{\rrbracket{}}\phiTerminal{,}\;\phiEOL{}
& \quad{} \quad{} \quad{}\textnormal{\texttt{i5}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\varphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{ireturn}}{} \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/8629FAA36B44FD784C11DFBB19BD9D30-86-phiquation.tex <==
[[ |j\textdollar{}Numbers| -> [[
  @ -> Q.class,
  version -> 61,
  access -> 33,
  supername ->
    "java/lang/Object",
  interfaces -> [[ ]],
  |j\textdollar{}object\char64init\char64| -> [[\dots]],
  |j\textdollar{}total| -> [[\dots]],
  |\highlight{j\textdollar{}total\textdollar{}0}| -> [[
    @ -> Q.method,
    access -> 4106,
    descriptor -> "(I)I",
    body -> [[
      @ -> Q.seq.of6,
      i2 -> [[ @ -> Q.iload, |v| -> 0 ]],
      i3 -> [[ @ -> Q.iload, |v| -> 0 ]],
      i4 -> [[ @ -> Q.imul ]],
      i5 -> [[ @ -> Q.ireturn ]] ]] ]] ]] ]]


==> _eolang/paper/phiq.tex <==
Q.method

==> _eolang/paper/phiquation.tex <==
[[ |j\textdollar{}Numbers| -> [[
  @ -> Q.class,
  version -> 61,
  access -> 33,
  supername ->
    "java/lang/Object",
  interfaces -> [[ ]],
  |j\textdollar{}object\char64init\char64| -> [[\dots]],
  |j\textdollar{}total| -> [[\dots]],
  |\highlight{j\textdollar{}total\textdollar{}0}| -> [[
    @ -> Q.method,
    access -> 4106,
    descriptor -> "(I)I",
    body -> [[
      @ -> Q.seq.of6,
      i2 -> [[ @ -> Q.iload, |v| -> 0 ]],
      i3 -> [[ @ -> Q.iload, |v| -> 0 ]],
      i4 -> [[ @ -> Q.imul ]],
      i5 -> [[ @ -> Q.ireturn ]] ]] ]] ]] ]]


==> tables/moller-jvms/seconds.tex <==
1,358\endinput

==> tables/moller-jvms/table.tex <==
\begin{tabularx}{\linewidth}{X|l>{\ttfamily}r>{\ttfamily}r|l>{\ttfamily}r>{\ttfamily\arraybackslash}r}
\toprule
Vendor & JVM & {\rmfamily Ratio} & {\rmfamily RSD} & JVM & {\rmfamily Ratio} & {\rmfamily RSD} \\
\midrule
    Corretto & 8.0.442 & \textcolor{DarkRed}{1.865} & 1.82\% & 24.0.2 & 0.832 & 1.04\% \\ 
    GraalVM & 17.0.12 & \textcolor{DarkGreen}{0.607} & 1.11\% & 26.ea.6 & \textcolor{DarkGreen}{0.556} & 0.95\% \\ 
    Java.net & 21.0.2 & 0.818 & 2.22\% & 26.ea.7 & 0.827 & 7.46\% \\ 
    Microsoft & 11.0.26 & 0.960 & 0.88\% & 21.0.8 & 0.820 & 1.87\% \\ 
    Oracle & 17.0.12 & 0.817 & 2.40\% & 24.0.2 & 0.833 & 1.27\% \\ 
    Temurin & 11.0.18 & 0.983 & 5.19\% & 24.0.2 & 0.837 & 1.36\% \\ 
    Tencent & 8.0.432 & \textcolor{DarkRed}{1.861} & 2.72\% & 21.0.7 & 0.830 & 1.48\% \\ 
    Zulu & 8.0.462 & \textcolor{DarkRed}{1.870} & 1.01\% & 24.0.2 & 0.830 & 1.17\% \\ 
\bottomrule
\end{tabularx}


==> tables/streamliner-vs-hone/seconds.tex <==
7,169\endinput

==> tables/streamliner-vs-hone/table.tex <==
\begin{tabularx}{\linewidth}{X|>{\ttfamily}r>{\ttfamily}r>{\ttfamily}r>{\ttfamily}r|>{\ttfamily}r>{\ttfamily}r>{\ttfamily}r>{\ttfamily\arraybackslash}r}
\toprule
Benchmark & \multicolumn{4}{c|}{Zulu 17.0.16}  & \multicolumn{4}{c}{Zulu 23.0.2} \\
  & {\scshape Strm} & \(\pm\)RSD & \hone{} & \(\pm\)RSD  & {\scshape Strm} & \(\pm\)RSD & \hone{} & \(\pm\)RSD\\
\midrule
  \texttt{allMatch} & \textcolor{DarkGreen}{0.125} & 13.89\% & 1.000 & 0.00\% & \textcolor{DarkGreen}{0.167} & 0.00\% & 1.000 & 0.00\%\\
  \texttt{count} & \textcolor{DarkGreen}{0.111} & 4.93\% & 1.000 & 8.22\% & \textcolor{DarkGreen}{0.200} & 0.00\% & 1.000 & 0.00\%\\
  \texttt{filterCount} & \textcolor{DarkRed}{2.072} & 0.41\% & 1.015 & 2.77\% & \textcolor{DarkRed}{2.045} & 2.07\% & 0.987 & 2.15\%\\
  \texttt{filterMapCount} & \textcolor{DarkRed}{2.134} & 2.68\% & 1.024 & 2.88\% & \textcolor{DarkRed}{2.121} & 1.64\% & 1.024 & 1.69\%\\
  \texttt{megamorphicFilters} & \textcolor{DarkGreen}{0.053} & 0.72\% & \textcolor{DarkGreen}{0.053} & 0.54\% & \textcolor{DarkGreen}{0.052} & 2.11\% & \textcolor{DarkGreen}{0.051} & 0.81\%\\
  \texttt{megamorphicMaps} & \textcolor{DarkGreen}{0.012} & 0.55\% & \textcolor{DarkGreen}{0.034} & 0.38\% & \textcolor{DarkGreen}{0.010} & 1.50\% & \textcolor{DarkGreen}{0.010} & 1.78\%\\
  \texttt{sum} & 0.998 & 0.75\% & 0.999 & 0.70\% & 0.989 & 0.59\% & 1.000 & 0.96\%\\
  \texttt{sumOfSquares} & \textcolor{DarkGreen}{0.294} & 0.57\% & 1.002 & 0.52\% & 1.001 & 0.96\% & 0.997 & 0.60\%\\
  \texttt{sumOfSquaresEven} & 1.018 & 0.46\% & 1.014 & 0.34\% & 0.987 & 3.35\% & 0.983 & 3.32\%\\
\bottomrule
\end{tabularx}


==> tikz/rules.tex <==
% SPDX-FileCopyrightText: Copyright (c) 2025-2026 Objectionary.com
% SPDX-License-Identifier: MIT

\catcode`\$=3\relax
\resizebox{.98\textwidth}{!}{

\begin{tikzpicture}
[node distance=2.2em,
pragma/.style={fill=red!5},
stage/.style={draw=none, font={}, text width=6em, align=center},
num/.style={font={\small\ttfamily}, draw=none},
every edge/.style={draw, -{Latex[length=.6em, width=.6em]}, line width=.1em},
every node/.style={minimum height=1.8em, font={\ttfamily}, draw, line width=.05em, anchor=east, outer sep=.3em}]

\pgfmathsetmacro{\dist}{3.8}

\node[anchor=west] (i1) {aload\_1};
  \node[num, anchor=east] at (i1.west) {1:};
\node[below=of i1.west, anchor=west] (i2) {invokestatic};
  \node[num, anchor=east] at (i2.west) {2:};
\node[below=of i2.west, anchor=west] (i3) {invokedynamic};
  \node[num, anchor=east] at (i3.west) {3:};
\node[below=of i3.west, anchor=west] (i4) {invokeinterface};
  \node[num, anchor=east] at (i4.west) {4:};
\node[below=of i4.west, anchor=west] (i5) {invokedynamic};
  \node[num, anchor=east] at (i5.west) {5:};
\node[below=of i5.west, anchor=west] (i6) {invokeinterface};
  \node[num, anchor=east] at (i6.west) {6:};
\node[below=of i6.west, anchor=west] (i7) {invokeinterface};
  \node[num, anchor=east] at (i7.west) {7:};
\node[below=of i7.west, anchor=west] (i8) {ireturn};
  \node[num, anchor=east] at (i8.west) {8:};

\node[fit=(i3) (i4), draw=none, inner sep=0, outer sep=0] (map) {};
\node[fit=(i5) (i6), draw=none, inner sep=0, outer sep=0] (filter) {};
\node[pragma, right=\dist of map.west, anchor=west] (i3a) {\(\Phi\).map};
\node[pragma, right=\dist of filter.west, anchor=west] (i5a) {\(\Phi\).filter};

\node[right=\dist of i1.west, anchor=west] (i1a) {aload\_1};
\node[right=\dist of i2.west, anchor=west] (i2a) {invokestatic};
\node[right=\dist of i7.west, anchor=west] (i7a) {invokeinterface};
\node[right=\dist of i8.west, anchor=west] (i8a) {ireturn};

\draw (i1.east) edge (i1a.west);
\draw (i2.east) edge (i2a.west);
\path
  let
    \p1 = ([xshift=.3em,yshift=-.4em]map.north east),
    \p2 = ([xshift=.3em,yshift=.4em]map.south east),
    \p3 = ($(\p1)!0.5!(\p2)$)
  in
    (\p1) edge[-] (\p2)
    (\p3) edge (i3a.west);
\path
  let
    \p1 = ([xshift=.3em,yshift=-.4em]filter.north east),
    \p2 = ([xshift=.3em,yshift=.4em]filter.south east),
    \p3 = ($(\p1)!0.5!(\p2)$)
  in
    (\p1) edge[-] (\p2)
    (\p3) edge (i5a.west);
\draw (i7.east) edge (i7a.west);
\draw (i8.east) edge (i8a.west);

\node[right=\dist of i1a.west, anchor=west] (i1b) {aload\_1};
\node[right=\dist of i2a.west, anchor=west] (i2b) {invokestatic};
\node[right=\dist of i7a.west, anchor=west] (i7b) {invokeinterface};
\node[right=\dist of i8a.west, anchor=west] (i8b) {ireturn};
\node[pragma, right=\dist of i3a.west, anchor=west] (i3b) {\(\Phi\).distill};
\node[pragma, right=\dist of i5a.west, anchor=west] (i5b) {\(\Phi\).distill};
\draw (i1a.east) edge (i1b.west);
\draw (i2a.east) edge (i2b.west);
\draw (i3a.east) edge (i3b.west);
\draw (i5a.east) edge (i5b.west);
\draw (i7a.east) edge (i7b.west);
\draw (i8a.east) edge (i8b.west);

\node[fit=(i3b) (i5b), draw=none, inner sep=0, outer sep=0] (distill) {};
\node[right=\dist of i1b.west, anchor=west] (i1c) {aload\_1};
\node[right=\dist of i2b.west, anchor=west] (i2c) {invokestatic};
\node[right=\dist of i7b.west, anchor=west] (i7c) {invokeinterface};
\node[right=\dist of i8b.west, anchor=west] (i8c) {ireturn};
\node[pragma, right=\dist of distill.west, anchor=west] (i3c) {\(\Phi\).distill};
\path
  let
    \p1 = ([xshift=.3em,yshift=-.4em]distill.north east),
    \p2 = ([xshift=.3em,yshift=.4em]distill.south east),
    \p3 = ($(\p1)!0.5!(\p2)$)
  in
    (\p1) edge[-] (\p2)
    (\p3) edge (i3c.west);
\draw (i1b.east) edge (i1c.west);
\draw (i2b.east) edge (i2c.west);
\draw (i7b.east) edge (i7c.west);
\draw (i8b.east) edge (i8c.west);

\node[right=\dist of i1c.west, anchor=west] (i1d) {aload\_1};
\node[right=\dist of i2c.west, anchor=west] (i2d) {invokestatic};
\node[right=\dist of i7c.west, anchor=west] (i7d) {invokeinterface};
\node[right=\dist of i8c.west, anchor=west] (i8d) {ireturn};
\node[pragma, right=\dist of i3c.west, anchor=west] (i3d) {\(\Phi\).mapMulti};
\draw (i1c.east) edge (i1d.west);
\draw (i2c.east) edge (i2d.west);
\draw (i3c.east) edge (i3d.west);
\draw (i7c.east) edge (i7d.west);
\draw (i8c.east) edge (i8d.west);

\pgfmathsetmacro{\edist}{5*\dist}
\node[right=\dist of i1d.west, anchor=west] (i1e) {aload\_1};
\node[right=\dist of i2d.west, anchor=west] (i2e) {invokestatic};
\node[right=\edist of i4.west, anchor=west] (i4e) {invokedynamic};
\node[right=\edist of i5.west, anchor=west] (i5e) {invokeinterface};
\node[right=\dist of i7d.west, anchor=west] (i7e) {invokeinterface};
\node[right=\dist of i8d.west, anchor=west] (i8e) {ireturn};
\draw (i1d.east) edge (i1e.west);
\draw (i2d.east) edge (i2e.west);
\draw (i7d.east) edge (i7e.west);
\draw (i8d.east) edge (i8e.west);
\path
  let
    \p1 = ([xshift=-2em]i4e.west),
    \p2 = ([xshift=-2em]i5e.west),
    \p3 = ($(\p1)!0.5!(\p2)$)
  in
    (i3d.east) edge[-] (\p3)
    (\p1) edge[-] (\p2)
    (\p1) edge (i4e.west)
    (\p2) edge (i5e.west);

\node[stage, anchor=north] at ([xshift=-1em, yshift=-1em] i8a.west) {1) Rewriting instructions to pragmas};
\node[stage, anchor=north] at ([xshift=-1em, yshift=-1em] i8b.west) {2) Rewriting mapping and filtering pragmas to distilling pragmas};
\node[stage, anchor=north] at ([xshift=-1em, yshift=-1em] i8c.west) {3) Merging distilling pragmas};
\node[stage, anchor=north] at ([xshift=-1em, yshift=-1em] i8d.west) {4) Rewriting distilling to mapMulti pragmas};
\node[stage, anchor=north] at ([xshift=-1em, yshift=-1em] i8e.west) {5) Rewriting pragmas to instructions};
\end{tikzpicture}

}
\catcode`\$=\active


==> tikz/workflow.tex <==
% SPDX-FileCopyrightText: Copyright (c) 2025-2026 Objectionary.com
% SPDX-License-Identifier: MIT

\begin{tikzpicture}
[node distance=1.8em,
every node/.style={draw, line width=.08em},
every edge/.style={draw, -{Latex[length=1em, width=.8em]}, line width=.1em},
tool/.style={draw=gray, label position=north west, fill=green!5, line width=.03em}]
\node[fill=blue!5] (sys) {
  \begin{tabular}{l>{\(\longrightarrow\)\;\arraybackslash}l}
    \texttt{invokedynamic} & \(\Phi\).\texttt{map} \\
    \texttt{invokedynamic} & \(\Phi\).\texttt{filter} \\
    \(\Phi\).\texttt{map} & \(\Phi\).\texttt{distill} \\
    \(\Phi\).\texttt{filter} & \(\Phi\).\texttt{distill} \\
    \highlight{\(\Phi\).\texttt{distill} + \(\Phi\).\texttt{distill}} & \highlight{\(\Phi\).\texttt{distill}} \\
    \(\Phi\).\texttt{distill} & \(\Phi\).\texttt{mapMulti} \\
    \(\Phi\).\texttt{mapMulti} & \texttt{invokedynamic} \\
    \(\Phi\).\texttt{map} & \texttt{invokedynamic} \\
    \(\Phi\).\texttt{filter} & \texttt{invokedynamic} \\
  \end{tabular}
};
\node[above=1.2 of sys] (phi1) {\parbox{7em}{\centering Original \(\varphi\)-expressions in \texttt{.phi} files}};
\node[below right=1.6 and -.5 of sys.south] (phi2) {\parbox{7em}{\centering Rewritten \(\varphi\)-expressions in \texttt{.phi} files}};
\begin{scope}[on background layer]
    \path (phi1) edge node[tool, very near end] {\phino} (phi2);
\end{scope}
\node[left=1.8 of phi1] (xmir1) {\parbox{5em}{\centering Original XMIR in \texttt{.xmir} files}};
\node[left=1.8 of xmir1] (bc1) {\parbox{6em}{\centering Original bytecode in \texttt{.class} files}};
\node[below=1.6 of bc1] (java) {\parbox{5em}{\centering Java source code in \texttt{.java} files}};
\path (java) edge node[tool] {\tool{javac}} (bc1);
\path (bc1) edge[bend right=45] node[tool] (jeo1) {\jeo} (xmir1);
\path (xmir1) edge[bend right=45] node[tool] (phino1) {\phino} (phi1);
\node[left=1.8 of phi2] (xmir2) {\parbox{5em}{\centering Optimized XMIR in \texttt{.xmir} files}};
\node[left=2 of xmir2] (bc2) {\parbox{6em}{\centering Optimized bytecode in \texttt{.class} files}};
\path (phi2) edge[bend right=45] node[tool] (phino2) {\phino} (xmir2);
\path (xmir2) edge[bend right=45] node[tool] (jeo2) {\jeo} (bc2);
\node [dashed, fit=(sys) (phino1) (phino2) (jeo1) (jeo2)] (hone) {};
\node [fill=red!5, anchor=north east, draw=none] at (hone.north east) {\hone{}};
\end{tikzpicture}

